RL from Physical Feedback: Aligning Large Motion Models with Humanoid Control

This paper focuses on a critical challenge in robotics: translating text-driven human motions into executable actions for humanoid robots, enabling efficient and cost-effective learning of new behaviors. While existing text-to-motion generation methods achieve semantic alignment between language and motion, they often produce kinematically or physically infeasible motions unsuitable for real-world deployment. To bridge this sim-to-real gap, we propose Reinforcement Learning from Physical Feedback (RLPF), a novel framework that integrates physics-aware motion evaluation with text-conditioned motion generation. RLPF employs a motion tracking policy to assess feasibility in a physics simulator, generating rewards for fine-tuning the motion generator. Furthermore, RLPF introduces an alignment verification module to preserve semantic fidelity to text instructions. This joint optimization ensures both physical plausibility and instruction alignment. Extensive experiments show that RLPF greatly outperforms baseline methods in generating physically feasible motions while maintaining semantic correspondence with text instruction, enabling successful deployment on real humanoid robots.

==> CMU_up_table.tex <==
\begin{table}[ht]
\centering
\caption{High-Level Generation Evaluation results on the CMU testset.}
\footnotesize
\label{tab:high-cmu}

\begin{tabular}{l|c ccc c}
\toprule
\textbf{Method} & 
{\textbf{FID ↓}} & 
{\textbf{R@1 ↑}} & 
{\textbf{R@2 ↑}} & 
{\textbf{R@3 ↑}} & 
{\textbf{MMDist ↓}} \\

\midrule

Base Model & \cellcolor{tablepeach}{\textcolor{black}{2.35}}  & 0.2375 & 0.3781 & 0.4906 & 4.1746 \\
SFT        & 3.18 & 0.2469 & 0.3938 & 0.4938 & 4.1139  \\
SFT-Filter   & 4.11  & 0.1938 & 0.3406 & 0.4563  & 4.2249    \\
\midrule
GT & -- & 0.29 &0.46  &0.58 &3.54 \\
\midrule
\textbf{RLPF-MA}   & 3.61  & \cellcolor{tablepeach}{\textcolor{black}{0.2594}} & \cellcolor{tablepeach}{\textcolor{black}{0.4188}} & \cellcolor{tablepeach}{\textcolor{black}{0.5563}}  & \cellcolor{tablepeach}{\textcolor{black}{3.6229}}  \\
\textbf{RLPF-TA}  & 8.23  & 0.2125 & 0.3813 & 0.5406  & 3.6518  \\
\bottomrule
\end{tabular}

\label{tab:cmu_results}
\end{table}


==> ablation1.tex <==
\begin{table}[ht]
\centering
\caption{Evaluation results on IsaacGym and MuJoCo test environments.}
\begin{tabular}{lccc|ccc}
\toprule
& \multicolumn{3}{c|}{\textbf{IsaacGym}} & \multicolumn{3}{c}{\textbf{MuJoCo}} \\
\cmidrule(lr){2-4}  \cmidrule(lr){5-7}
\textbf{Method} & 
\textcolor{darkblue}{\textbf{sr ↑}} & 
\textcolor{darkblue}{\textbf{mpjpe ↓}} & 
\textcolor{darkblue}{\textbf{mpkpe ↓}} & 
\textcolor{darkgreen}{\textbf{sr ↑}} & 
\textcolor{darkgreen}{\textbf{mpjpe ↓}} & 
\textcolor{darkgreen}{\textbf{mpkpe ↓}} \\
\midrule
MA                 & 0.9195 & 0.1793 & 0.1283 & 0.6307 & 0.280 & 0.4621 \\
TA                 & 0.8950 & 0.1903 & 0.1518 & 0.6610 & 0.280 & 0.2799 \\
RLPF-PHC-MA        & 0.9075 & 0.1772 & 0.1386 & 0.6502 & 0.270 & 0.3272 \\
RLPF-PHC-TA        & 0.7512 & 0.1797 & 0.1418 & 0.6071 & 0.290 & 0.4454 \\
RLPF-w/o align     & 0.9062 & 0.1835 & 0.1182 & 0.9014 & 0.290 & 0.1870 \\
\bottomrule
\end{tabular}
\label{tab:isaac_mujoco_comparison}
\end{table}


==> amass_up_table.tex <==
\begin{table}[ht]
\centering
\caption{High-Level Generation Evaluation results on the AMASS testset.}
\begin{tabular}{l|ccccc}
\toprule
\textbf{Method} & 
{\textbf{FID ↓}} & 
{\textbf{R@1 ↑}} & 
{\textbf{R@2 ↑}} & 
{\textbf{R@3 ↑}} & 
{\textbf{MMDist ↓}} \\
\midrule
Base Model                \cellcolor{tablepeach}{\textcolor{black}{ 1.79}} & 0.22 & 0.35 & 0.46 & 4.62   \\
SFT                & 1.79 & 0.22 & 0.35 & 0.46 & 4.62   \\
SFT\_Filter    & 3.09 & 0.23 & 0.40 & 0.51 & 4.21  \\
\midrule
GT                  & --    & 0.37 & 0.58 & 0.67 & 3.23   \\
\midrule
\textbf{RLPF-MA}            & 3.34 & \cellcolor{tablepeach}{\textcolor{black}{ 0.27}} & 0.45 & 0.57 & 3.75   \\
\textbf{RLPF-TA}         & 4.47 & 0.26 & 0.41 & 0.52 & 3.70   \\
\bottomrule
\end{tabular}
\label{tab:cmu_partial_results}
\end{table}


==> main-up.tex <==
\begin{table}[ht]
\centering
\caption{High-Level Generation Evaluation results on both CMU and AMASS testset.}
\label{tab:high}
\begin{tabular}{lcccccc}
\toprule
 & 
\multicolumn{3}{c}{\textcolor{darkblue}{\textbf{CMU}}} & 
\multicolumn{3}{c}{\textcolor{darkgreen}{\textbf{AMASS}}} \\
\cmidrule(lr){2-4}  \cmidrule(lr){5-7}
\textbf{Method}& {\textbf{$FID$ ↓}} & 
  {\textbf{$R@1$ ↑}} & 
  {\textbf{$R@2$ ↑}} & 
  {\textbf{$R@3$ ↑}} & 
  {\textbf{$MMDist$ ↓}} & 
  {\textbf{$FID$ ↓}} & 
  {\textbf{$R@1$ ↑}} & 
  {\textbf{$R@2$ ↑}} & 
  {\textbf{$R@3$ ↑}} & 
  {\textbf{$MMDist$ ↓}}\\
\midrule
Base Model                & \cellcolor{tablepeach}{\textcolor{black}{2.35}}  & 0.2375 & 0.3781 & 0.4906 & 4.1746 & 1.79 & 0.22 & 0.35 & 0.46 & 4.62 \\
SFT           & 3.18 & 0.2469 & 0.3938 & 0.4938 & 4.1139 & \cellcolor{tablepeach}{\textcolor{black}{ 1.79}} & 0.22 & 0.35 & 0.46 & 4.62 \\
SFT-Filter   & 4.11  & 0.1938 & 0.3406 & 0.4563  & 4.2249 & 3.09 & 0.23 & 0.40 & 0.51 & 4.21 \\
\midrule
GT & -- & 0.29 &0.46  &0.58 &3.54 & --    & 0.37 & 0.58 & 0.67 & 3.23 \\
\midrule
\textbf{RLPF-MA}           &  3.61  & \cellcolor{tablepeach}{\textcolor{black}{0.2594}} & \cellcolor{tablepeach}{\textcolor{black}{0.4188}} & \cellcolor{tablepeach}{\textcolor{black}{0.5563}}  & \cellcolor{tablepeach}{\textcolor{black}{3.6229}} & 3.34 & \cellcolor{tablepeach}{\textcolor{black}{ 0.27}} & \cellcolor{tablepeach}{\textcolor{black}{ 0.45}} &\cellcolor{tablepeach}{\textcolor{black}{ 0.57}} & 3.75   \\
\textbf{RLPF-TA}           & 8.23  & 0.2125 & 0.3813 & 0.5406  & 3.6518  & 4.47 & 0.26 & 0.41 & 0.52 & 3.70  \\
\bottomrule
\end{tabular}
\label{tab:main-up}
\end{table}


==> sec_bak/0_abstract.tex <==
\begin{figure}[ht]
    \centering
    % \vspace{-4mm}
    \includegraphics[width=.9\linewidth]{fig/first_fig.pdf}
    \caption{Different behaviors of traditional text-to-motion models and our proposed RLPF in simulated and on real robots. The results show that the motion generated by the traditional text-to-motion generation models is not conducive to simulation and real machine deployment, while RLPF satisfies the semantic consistency of text and motion while ensuring physical feasibility and deployment capabilities.}
    \label{fig:first_fig}
    % \vspace{-4pt}
\end{figure}

\begin{abstract}
Text-to-motion generation builds a bridge between text instructions and humanoid robot actions.
Existing studies have primarily focused on the semantic correspondence of generated motions. 
However, in practice, generated motions from these methods often suffer from significant physical inconsistency, hindering their deployment in real humanoid robots.
To address this issue, we propose a novel learning framework--\textbf{Reinforcement Learning from Physical Feedback (RLPF)}.
Our approach leverages a pre-trained motion tracking policy to assess the feasibility of generated motions in a physics simulator.
Additionally, it incorporates an alignment verification module to guide the generation of motions that closely adhere to the input instructions. We then fine-tune the large motion model to jointly optimize these two objectives via reinforcement learning.
Experimental results demonstrate that RLPF greatly enhances the physical feasibility of motions generated by the large motion model while maintaining the semantic correspondence. 
  % Text-to-motion generation, a pivotal task in computer-aided content creation, has recently attracted increasing research interest and shows significant potential for applications in robotics.
  % Existing studies have primarily focused on improving numerical performance metrics on benchmark datasets.
  % However, in practical scenarios, generated motions often exhibit significant physical inconsistencies, resulting in distortions that hinder their seamless deployment in real-world applications.
  % To address this issue, we propose an innovative method called "RL from Physical Feedback."
  % Our approach leverages a pre-trained motion tracker to critique the generated motions, allowing for the assessment of their physical plausibility.
  % Additionally, it integrates a text-motion alignment reward model to guide the generation of motions that closely align with the input text.
  % Experimental results confirm the effectiveness of the proposed approach.
\end{abstract}

==> sec_bak/1_intro.tex <==


\section{Introduction}
\label{sec:intro}

For decades, the idea of creating lifelike characters that mimic human behavior --- capable of serving as partners in both virtual and physical worlds --- has been a compelling vision. 
This aspiration has gained significant momentum in recent years, fueled by breakthroughs in humanoid robot hardware. 
With increasing degrees of freedom (DoF) and reliability of hardware, these robots (e.g., Unitree G1, Tesla Optimus) can now perform remarkably fluid motions, such as dancing, which were impossible to achieve before.
Unfortunately, this progress comes with significant challenges, where each motion relies on labor-intensive parameter tuning, severely limiting scalability across diverse actions.

%However, generating such motions traditionally requires labor-intensive manual tuning of parameters, making it impractical to scale to diverse actions.

This fundamental constraint has driven substantial interest in automated solutions, particularly text-to-motion (T2M) generation~\cite{lin2023motion}, which formally defines motion as temporal sequences of joint positions and rotations representing a character's spatial movement.
Existing T2M models offer promising capabilities, producing diverse human motions that can serve as valuable prior knowledge for humanoid robots to learn.
Recently, the integration of large language models (LLMs)~\citep{touvron2023open} has further transformed T2M models into large motion models, enabling more generalizable and human-aligned motion generation that better interprets user intent~\citep{wang2024motiongpt,wang2024quo}.
Yet despite these advances, a crucial question persists: \textit{Do current large motion models genuinely achieve our original aspiration of creating humanoid robots capable of performing the full spectrum of human-like motions with natural fluidity?}


Unfortunately, the answer is \textbf{NO}.
Current large motion models fall short of this goal. 
A significant gap remains between the motions generated by large motion models and those executable by humanoid robots, necessitating advanced motion tracking policies~\citep{ji2024exbody2} to bridge text-guided human motions with physically feasible robot actions. 
This limitation stems from the origins of current human motion research.
Most recent text-to-motion generation studies~\citep{zhang2024motiondiffuse, azadi2023make} have emerged from computer graphics, virtual reality, and gaming applications.  
While these works have made impressive progress in achieving semantic correspondence between text and motion, they frequently overlook a critical requirement for robotics: \textbf{physical feasibility}. 
The generated motions often violate physical constraints or fail to account for the dynamic stability requirements essential for real-world humanoid robot deployment.
In short, this paper focuses on investigating the following question:


\begin{center}

\textbf{\textit{How can we align large motion models with whole-body control systems for humanoid robots,\\ensuring generated motions maintain both semantic correspondence and physical feasibility?
}}
    
\end{center}
%How can we align large motion model based motion generator with humanoid robot whole body control?


To achieve this, we must enhance large motion models to produce physically feasible outputs.
Physical feasibility encompasses several critical factors:
\textbf{i) Morphological Adaptation. } 
The inherent morphological differences between human bodies and humanoid robots make direct motion transfer impractical, requiring sophisticated motion retargeting techniques to achieve functional equivalence while respecting robotic kinematic constraints.
\textbf{ii) Physical Consistency. }
Current models typically generate motions containing artifacts like foot sliding, ground penetration~\citep{yuan2023physdiff, han2025reindiffuse, tseng2023edge}, and unnatural body dynamics.
These artifacts not only break physical laws but also cause catastrophic execution failures in real robot systems.
The two challenges highlight the importance of incorporating physical feasibility throughout motion generation for humanoid robot applications.

%Firstly, due to morphological differences between the human body and humanoid robots, direct transfer of motion is often infeasible, necessitating a motion retargeting process. In addition, the generated motions frequently exhibit physical inconsistencies such as foot sliding, ground penetration~\citep{yuan2023physdiff, han2025reindiffuse, tseng2023edge}, or unnatural body dynamics. These artifacts cause execution failures in real-world robotic systems. These aforementioned two challenges collectively highlight the importance of ensuring physical feasibility in motion generation, especially for humanoid robots.




To tackle these challenges, we propose a novel reinforcement learning (RL) framework for fine-tuning large motion model to ensure physical feasibility.
Our approach consists of three key components:
\textbf{i) Motion Tracking Policy.}
We develop a robust motion tracker based on Exbody2~\citep{ji2024exbody2}, enabling humanoid robots to precisely execute reference motions while providing a signal of physical feasibility.
%Concretely, we train a motion tracking policy based on Exbody2~\citep{ji2024exbody2}, enabling humanoid robots to accurately follow reference motions and serving as a signal of physical feasibility. 
\textbf{ii) Alignment Verification Module.}
We introduce this verification module that evaluates semantic correspondence feedback between generated motions and their textual instruction.
%Additionally, we introduce an alignment verification module to provide the signal of the semantic correspondence of generated motions. 
\textbf{iii) RL-based Finetuning.}
We employ a RL framework to optimize the large motion model using both physical feasibility signals from the tracking policy and semantic alignment feedback from the verification module.
%Subsequently, we further fine-tune the motion generator with reinforcement learning to enhance the feasibility of generated motions using both the above signals. 
%Experiments demonstrate our approach achieves both physical feasibility and semantic correspondence of generated motions.
%achieves both physical feasibility and semantic correspondence of generated motions.


%To tackle these challenges, we propose a novel approach that fine-tunes motion generators via reinforcement learning to produce physically feasible motions. Concretely, we train a motion tracking policy based on Exbody2~\citep{ji2024exbody2}, enabling humanoid robots to accurately follow reference motions and serving as a signal of physical feasibility. Additionally, we introduce an alignment verification module to provide the signal of the semantic correspondence of generated motions. Subsequently, we further fine-tune the motion generator with reinforcement learning to enhance the feasibility of generated motions using both the above signals. Experimental results validate our method achieves both physical feasibility and semantic correspondence of generated motions.


In summary, our contributions are threefold: 
\begin{itemize}
\item We propose \textbf{Reinforcement Learning from Physical Feedback (RLPF)}, a novel reinforcement learning framework that optimizes large motion models to greatly enhance physical feasibility of generated motions, with the help of a motion tracking policy. 
\item We introduce an alignment verification module that quantitatively evaluates semantic correspondence, enabling RLPF to maintain semantic alignment while avoiding conservative motion generation that compromises action expressiveness.
\item Through extensive experiments, we demonstrate that our approach significantly improves physical feasibility while maintaining strong semantic alignment with the generated motions. 
These results highlight the potential of our framework for bridging the gap between text-to-motion generation and real-world humanoid whole-body control.
\end{itemize}


  
% Experimental results validate the effectiveness of our approach. First, the generated motions show significant improvements in physical feasibility, as evidenced by higher success rates of the motion tracking policy and improved metrics such as MPJPE. Second, the generated motions maintain alignment with the input text, as reflected in metrics like Fréchet Inception Distance (FID) and retrieval accuracy. These results demonstrate that our method can generate motion sequences that are both physically executable and consistently aligned with textual instructions, providing a reliable solution for training and deploying humanoid robots.

% Our reinforcement learning fine-tuning framework incorporates two critical reward functions. The first is a motion tracking reward, which assesses the physical feasibility of generated motions by executing them through the motion tracking policy and quantifying positional deviations of key body joints, including both Mean Per Keypoint Position Error (MPKPE) and Mean Per Joint Position Error (MPJPE). The second is an alignment reward, which ensures the generated motions maintain semantic consistency with the input text description. This is achieved by leveraging a pre-trained, frozen text-motion retrieval model to evaluate the motion-text correspondence. Both reward functions remain fixed during training, eliminating the need for additional fine-tuning and thereby enhancing training efficiency.






%Prior work has proposed leveraging the relatively abundant human motion data to synthesize motion sequences using large-scale motion generation models trained on diverse textual descriptions. These models, such as MotionGPT~\citep{jiang2023motiongpt}, treat human motion as a "foreign language", generating diverse and complex sequences from textual input through a unified vocabulary, thus serving as valuable data generators for robot training.

%Text-to-motion generation bridges the gap between text instruction and humanoid robot actions. However, 
%\yu{The progress of humanoid robotics is hindered by the shortage of high-quality training data, which is crucial for developing advanced control strategies.}
%\del{The advancement of humanoid robotics is impeded by the lack of high-quality training data, which is essential for developing sophisticated control strategies.}Prior work has proposed leveraging the relatively abundant human motion data to synthesize motion sequences using large-scale motion generation models trained on diverse textual descriptions. These models, such as MotionGPT~\citep{jiang2023motiongpt}, treat human motion as a "foreign language", generating diverse and complex sequences from textual input through a unified vocabulary, thus serving as valuable data generators for robot training.

%However, applying these generated human motions directly to humanoid robots poses several significant challenges. Due to morphological differences between the human body and humanoid robots, direct transfer of motion is often infeasible, necessitating a motion retargeting process. To address this, optimization-based retargeting methods are commonly employed, which minimize the distance between corresponding points on the human and robot models while incorporating regularization terms to ensure motion naturalness and smoothness.
%In addition, the generated motions frequently exhibit physical inconsistencies such as foot sliding, ground penetration, or unnatural body dynamics. These artifacts not only reduce the realism of the motion but also cause execution failures in real-world robotic systems.
%Moreover, a single textual command may correspond to multiple plausible motion sequences—reflecting the inherent one-to-many mapping between language and motion. However, not all such sequences are compatible with a robot’s kinematic and dynamic constraints. For instance, in response to a command like “walk forward”, a generated motion with an overly slow pace may lead to loss of balance during leg lift, whereas an excessively fast pace may exceed the robot’s control bandwidth, increasing the difficulty of accurate tracking and execution.

% However, applying these generated human motions directly to robots presents several challenges. Firstly, the generated motions may exhibit physical inconsistencies—such as floating, skating, or penetration, which are unrealistic and lead to execution failures. Secondly, a single textual description may correspond to multiple motion sequences (a one-to-many mapping), though not all are feasible due to the kinematic and dynamic constraints of robots. For instance, in response to a “walk forward” command, if the pace is too slow, the robot may lose balance while lifting its foot; if too fast, it may struggle to follow accurately, complicating the learning process. Furthermore, adapting human motion data for robots necessitates motion retargeting. An optimization-based retargeting method is typically adopted, which minimizes the distance between corresponding points on the human and robot models while incorporating regularization terms to preserve motion naturalness and smoothness.

% To address these issues, we propose a novel approach that fine-tunes motion generation models through reinforcement learning to produce motion sequences that are both physically consistent.Concurrently, we train a motion tracking policy based on the Perpetual Humanoid Control (PHC) framework~\citep{luo2023perpetual}, enabling the robot to accurately follow generated motion sequences. Subsequently, we fine-tune the motion generator using reinforcement learning to ensure that the upstream motions are more readily executable by robots.

%To tackle these challenges, we propose a novel approach that fine-tunes motion generation models via reinforcement learning to produce physically consistent motion sequences. Concurrently, we train a motion tracking policy based on the Perpetual Humanoid Control (PHC) framework~\citep{luo2023perpetual}, enabling robots to accurately follow the generated sequences. Subsequently, we further fine-tune the motion generator with reinforcement learning to enhance the executability of upstream motions by robots.

% Our reinforcement learning fine-tuning approach employs two key reward functions. The first is a motion tracking reward, which evaluates the physical executability of generated motions by feeding them into the motion tracking policy and measuring errors in position of key points (e.g., Mean Per Keypoint Position Error, MPKPE) and MPJPE during tracking. The second is an alignment reward, which constrains the motion generator from deviating from the semantic consistency of the input text. We use a frozen text-motion retrieval model to assess the alignment between generated motions and input text. Both reward functions are frozen, requiring no further fine-tuning, thus improving training efficiency.

%Our reinforcement learning fine-tuning framework incorporates two critical reward functions. The first is a motion tracking reward, which assesses the physical feasibility of generated motions by executing them through the motion tracking policy and quantifying positional deviations of key body joints, including both Mean Per Keypoint Position Error (MPKPE) and Mean Per Joint Position Error (MPJPE). The second is an alignment reward, which ensures the generated motions maintain semantic consistency with the input text description. This is achieved by leveraging a pre-trained, frozen text-motion retrieval model to evaluate the motion-text correspondence. Both reward functions remain fixed during training, eliminating the need for additional fine-tuning and thereby enhancing training efficiency.

% plausibility

%Experimental results validate the effectiveness of our approach. First, the generated human motions show significant improvements in physical plausibility, as evidenced by higher success rates of the motion tracking policy and improved metrics such as MPJPE. Second, the generated motions maintain alignment with the input text, as reflected in metrics like Fréchet Inception Distance (FID) and retrieval accuracy. These results demonstrate that our method can generate motion sequences that are both physically executable and consistently aligned with textual instructions, providing a reliable solution for training and deploying humanoid robots.

% Related work has laid the foundation for our research. For instance, WHAM~\citep{shin2024wham} demonstrates the potential of extracting human motion data from third-person perspective videos, leveraging internet video data. CloSD~\citep{tevet2024closd} achieves text-driven hierarchical motion planning by combining a diffusion-based upstream planner with a frozen PHC motion tracking policy. Building on these efforts, our approach further enhances the practicality of generated motions for robotic applications through physical feedback and reinforcement learning optimization.

% In summary, our method bridges the gap between human motion generation and humanoid robot control by generating physically plausible and text-aligned motion sequences, offering a viable path for robot training and real-world deployment.

%In Summary, our contributions are threefold: 1) We propose a novel reinforcement learning framework, \textbf{Reinforcement Learning from Physical Feedback (RLPF)}, which fine-tunes motion generation models by using tracking performance as a reward signal. This approach innovatively leverages execution quality, which is measured by how accurately a pretrained motion tracking policy follows the generated motion, as direct feedback to guide the motion generator to produce physically plausible outputs. 2) To prevent the generator from overfitting to conservative motions that sacrifice semantic fidelity, we introduce a \textbf{text-motion alignment reward}. This reward is computed using a frozen, pretrained text-motion retrieval model, ensuring that the generated motion remains semantically consistent with the original textual instruction throughout the optimization process. 3) We conduct extensive experiments demonstrating that our approach significantly improves \textbf{physical executability} while maintaining strong \textbf{semantic consistency} with the input instructions. These results highlight the potential of our framework for bridging the gap between text-to-motion generation and real-world humanoid whole body control.

% \begin{itemize}[topsep=0.5pt, partopsep=0.5pt, itemsep=1pt, parsep=0.5pt]
%     \item \textbf{We propose a novel reinforcement learning framework, termed Reinforcement Learning from Physical Feedback, which fine-tunes motion generation models using tracking performance as a reward signal.} 
    
%     This approach innovatively leverages execution quality, which is measured by how accurately a pretrained motion tracking policy follows the generated motion, as direct feedback to guide the motion generator to produce physically plausible outputs.

%     \item \textbf{To prevent the generator from overfitting to conservative motions that sacrifice semantic fidelity, we introduce a text-motion alignment reward.}
    
%     This reward is computed using a frozen, pretrained text-motion retrieval model, ensuring that the generated motion remains semantically consistent with the original textual instruction throughout the optimization process.

%     \item \textbf{Extensive experiments validate the effectiveness of our method, demonstrating significant improvements in physical executability while maintaining strong semantic alignment with the input instructions.} 
    
%     These results highlight the potential of our framework for bridging the gap between text-to-motion generation and real-world humanoid whole body control.
% \end{itemize}



% Moreover, a single text instruction may correspond to multiple plausible motion sequences—reflecting the inherent one-to-many mapping between language and motion. However, not all such sequences are compatible with a robot’s kinematic and dynamic constraints. For instance, in response to a command like “walk forward”, a generated motion with an overly slow pace may lead to loss of balance during leg lift, whereas an excessively fast pace may exceed the robot’s control bandwidth, increasing the difficulty of accurate tracking and execution.

%The progress of humanoid robotics is hindered by the shortage of paired text-action data. One way to alleviate such a shortage is to build a pipeline consisting of a text-to-motion generator and a motion tracking policy so that we can bridge text instructions, human motions, and humanoid actions. While motion tracking policies are generally designed for humanoid robots, the studies about text-to-motion generation mostly originated from Computer Graphics, VR, Games, etc~\citep{zhang2024motiondiffuse, azadi2023make}. These works have primarily focused on the semantic correspondence of generated motions. However, they often neglect the physical feasibility, which is crucial for deploying the generated motion in humanoid robots.

%To achieve this, we are required to enable large motion models with physical-feasible outputThe physical feasibility could be related to several factors.Firstly, due to morphological differences between the human body and humanoid robots, direct transfer of motion is often infeasible, necessitating a motion retargeting process.In addition, the generated motions frequently exhibit physical inconsistencies such as foot sliding, ground penetration~\citep{yuan2023physdiff, han2025reindiffuse, tseng2023edge}, or unnatural body dynamics. These artifacts cause execution failures in real-world robotic systems. These aforementioned two challenges collectively highlight the importance of ensuring physical feasibility in motion generation, especially for humanoid robots.


    % This approach innovatively leverages execution quality, which is measured by how accurately a pretrained motion tracking policy follows the generated motion, as direct feedback to guide the motion generator to produce physically plausible outputs.
    % This reward is computed using a frozen, pretrained text-motion retrieval model, ensuring that the generated motion remains semantically consistent with the original textual instruction throughout the optimization process.

==> sec_bak/3_method.tex <==

\section{RL from Physical Feedback}
\label{sec:method}

% \begin{figure}[ht]
%     \centering
%     % \vspace{-4mm}
%     \includegraphics[width=.95\linewidth]{fig/RLPF_method.pdf}
%     \caption{Overview of RLPF}
%     \label{fig:method}
%     \vspace{-4pt}
% \end{figure}

\begin{figure}[ht]
    \centering
    % \vspace{-4mm}
    \includegraphics[width=1\linewidth]{fig/RLPF.pdf}
    \caption{Overview of RLPF. RLPF consists of three key components: (i) A motion tracking policy is pre-trained to develop a motion tracking reward for the generated motions; (ii) An alignment verification module is proposed for improving the consistency between input text semantics and generated motion while maintaining physically plausible; (iii) We use the RL framework to assist in optimizing the physical feasibility and semantic consistency of motions generated by the large motion model.
    }
    \label{fig:method}
    % \vspace{-2mm}
\end{figure}   

\subsection{Large Motion Model Pre-Training}
\subsubsection{Motion Tokenizer}

Similar to previous large motion models~\citep{jiang2023motiongpt}, to enable Large Language Models (LLMs) to understand and generate continuous motion features, we treat motion as a "foreign language" and employ a motion tokenizer built upon the VQ-VAE framework~\citep{van2017neural} to translate motion features into motion tokens. The motion tokenizer consists of an encoder $\mathcal{E}$ and a decoder $\mathcal{D}$, which encodes a $M$ frame motion $\Vec{m}_{1:M} = \{ m_i \}_{i=1}^M$ into $L$ motion tokens $\Vec{z}_{1:L} = \{ z_i \}_{i=1}^L$, and decodes $\Vec{z}_{1:L}$ back into the motion $\Vec{m}_{1:M} = \mathcal{D}(\Vec{z}_{1:L}) = \mathcal{D}(\mathcal{E}(\Vec{m}_{1:M}))$. 

% Similar to previous large motion models~\citep{jiang2023motiongpt}, we treat motion as a "foreign language" and employ a motion tokenizer built upon the VQ-VAE framework~\citep{van2017neural} to translate motion clip features into motion tokens.

% To enable Large Language Models (LLMs) to understand and generate continuous motion features, we employed a motion tokenizer to discretize these features. The motion tokenizer consists of an encoder $\mathcal{E}$ and a decoder $\mathcal{D}$, which encodes a $M$ frame motion $\Vec{m}^{1:M} = \{ m^i \}_{i=1}^M$ into $L$ motion tokens $\Vec{z}^{1:N} = \{ z^i \}_{i=1}^N$, and decodes $\Vec{z}^{1:L}$ back into the motion $\Vec{m}^{1:M} = \mathcal{D}(\Vec{z}^{1:L}) = \mathcal{D}(\mathcal{E}(\Vec{m}^{1:M}))$. 

\subsubsection{LLM-based Text-to-Motion Generator Pre-training}

By employing a motion tokenizer, the LLM backbone is empowered to understand and generate motion features. Specifically, we incorporate $K$ discrete codes from the motion codebook as an extension to the LLM's existing vocabulary.

The LLM backbone $\Theta$ is built on a decoder-only architecture using causal transformers. 
The LLM backbone first receives the provided text input tokens $\mathcal{L}$, based on which the model generates motion tokens $\Vec{z}_{1:L} = \{ z_i \}_{i=1}^L$ in an auto-regressive manner.
% The model generates motion tokens $\Vec{z}^{1:N} = \{ z^i \}_{i=1}^N$ in an auto-regressive manner, where 
Before the RL post-training, we first pre-train the motion generator in a large-scale text-motion dataset.
To train our model, we optimize the negative log-likelihood over the predicted tokens, which is defined as follows:
\[
% \begin{equation}
    \mathcal{L}(\Theta)=-\sum_{j=1}^{T} \log P_{\Theta}(z_j|l, \Vec{z}_{1:j-1}),
% \end{equation}
\]
where $l$, $\Vec{z}$, and $z$ denote the text instruction, generated token sequence and target token sequence, respectively. $\Theta$ represents the model parameters and $T$ is the length of the target sequence.

% $\mathcal{M}$ corresponds to the generated motion sequence based on the provided text input tokens $\mathcal{L}$.
% In this work, each text-motion pair in the dataset is framed as an instruction-following instance $\{\mathcal{L}, \mathcal{M}\}$, representing a question-answer interaction between the user and the motion model. 
% The entire instructional dataset adheres to this unified format.
% To train our model, we optimize the negative log-likelihood over the predicted tokens which is defined as follows:
% \begin{equation}
%     \mathcal{L}(\Theta)=-\sum_{j=1}^{T} \log P_{\Theta}(m_j|l, \hat{m}_{1:j-1}),
% \end{equation}
% %$\mathcal{Y}$ corresponds to the generated motion sequence.
% where $\hat{m}$ and $m$ denote the input and target token sequences, respectively. $\Theta$ represents the model parameters, $l$ is the input text description, and $T$ is the length of the target sequence.


% Specifically, our large motion model, built on a pre-trained LLM, functions as a generative model that connects a motion tokenizer with the LLM backbone $\Theta$. 
% The motion tokenizer encodes raw motion clip features $\mathcal{M}$ into motion tokens $\mathcal{z}=\{z_1,z_2,...,z_n\} \in \mathbbm{R}^{n \times d}$, where $n$ denotes the number of motion tokens and $d$ represents the dimensionality of each token.
% To integrate motion tokens into the LLM framework, we incorporate $K$ discrete codes in the motion codebook as additional vocabulary for the LLM.
% %we map the least frequently used $K$ tokens from the original LLM codebook to the motion codebook.
% Additionally, we introduce two special tokens, $<$mot$>$ and $<$/mot$>$, to signify the start and end of motion sequences within the input/output streams.
% The LLM backbone $\Theta$ is built on a decoder-only architecture using causal transformers. 
% The model generates motion tokens $\mathcal{M}=\{m_1,m_2,...,m_t\}$ in an auto-regressive manner, where $\mathcal{M}$ corresponds to the generated motion sequence based on the provided text input tokens $\mathcal{L}$.
% In this work, each text-motion pair in the dataset is framed as an instruction-following instance $\{\mathcal{L}, \mathcal{M}\}$, representing a question-answer interaction between the user and the motion model. 
% The entire instructional dataset adheres to this unified format.
% To train our model, we optimize the negative log-likelihood over the predicted tokens which is defined as follows:
% \begin{equation}
%     \mathcal{L}(\Theta)=-\sum_{j=1}^{T} \log P_{\Theta}(m_j|l, \hat{m}_{1:j-1}),
% \end{equation}
% %$\mathcal{Y}$ corresponds to the generated motion sequence.
% where $\hat{m}$ and $m$ denote the input and target token sequences, respectively. $\Theta$ represents the model parameters, $l$ is the input text description, and $T$ is the length of the target sequence.


\subsection{RL Fine-Tuning Motion Generator}

After pre-training the vanilla motion generator, we employ RL to finetune this model, enhancing both the physical feasibility and semantic correspondence of generated motions.
We formulate the motion generator as an actor policy \( \pi_\theta \), and finetune it using Group Relative Policy Optimization (GRPO) --- an RL algorithm that elimilates the need for a critic model and estimates the baseline from group scores instead, offering an advantage over standard PPO.

% Specifically, for each text instruction \( l \), GRPO samples a group of outputs \( \{\vec{m}^1, \vec{m}^2, \dots, \vec{m}^G\} \) from the old policy \( \pi_{\theta_{\text{old}}} \) and then optimizes the policy model \( \pi_\theta \) by maximizing the following objective:

% \[
% \frac{1}{G} \sum_{i=1}^G \left[ \min \left( \frac{\pi_\theta(\vec{m}^i|l)}{\pi_{\theta_{\text{old}}}(\vec{m}^i|l)} A_i, \text{clip} \left( \frac{\pi_\theta(\vec{m}^i|l)}{\pi_{\theta_{\text{old}}}(\vec{m}^i|l)}, 1 - \epsilon, 1 + \epsilon \right) A_i \right) - \beta \text{D}_{\text{KL}}(\pi_\theta \| \pi_{\text{ref}}) \right],
% \]

% \begin{flalign}
% &\mathcal{J}_{\text{GRPO}}(\theta) = \mathbb{E}\left[ l \sim P(L), \{\vec{m}^i\}_{i=1}^G \sim \pi_{\theta_{\text{old}}}(M|l) \right] \Bigg[ & \notag \\
% & \frac{1}{G} \sum_{i=1}^G \left[ \min \left( \frac{\pi_\theta(\vec{m}^i|l)}{\pi_{\theta_{\text{old}}}(\vec{m}^i|l)} A_i, \ \text{clip} \left( \frac{\pi_\theta(\vec{m}^i|l)}{\pi_{\theta_{\text{old}}}(\vec{m}^i|l)}, 1-\epsilon, 1+\epsilon \right) A_i \right) \right. & \notag \\
% & \left. - \beta \text{D}_{\text{KL}}(\pi_\theta \| \pi_{\text{ref}}) \right] \Bigg], & \notag \\
% &\text{where} \quad \text{D}_{\text{KL}}(\pi_\theta \| \pi_{\text{ref}}) = \mathbb{E}_{\pi_\theta} \left[ \log \frac{\pi_\theta(m|l)}{\pi_{\text{ref}}(m|l)} \right]. &
% \end{flalign}

% where \( \epsilon \) and \( \beta \) are hyper-parameters, and \( A_i \) is the advantage, computed using a group of rewards \( \{r_1, r_2, \dots, r_G\} \) corresponding to the outputs within each group:

% \[
% A_i = \frac{r_i - \text{mean}(\{r_1, r_2, \dots, r_G\})}{\text{std}(\{r_1, r_2, \dots, r_G\})}.
% \]



For each text instruction $l$, GRPO samples a group of generated motion tokens $Z = \{\vec{z}^1, \vec{z}^2, \dots, \vec{z}^G\}$ from the old policy $\pi_{\theta_{old}}$ and optimizes the policy model $\pi_{\theta}$ by maximizing the following objective:
\[
\footnotesize
\begin{split}
    \mathcal{J}_{GRPO}(\theta) &= \mathbb{E}{[l \sim P(L), \{\vec{z}^i\}_{i=1}^G \sim \pi_{\theta_{old}}(Z|l)]}  \\
    & \frac{1}{G}\sum_{i=1}^G \left( \min \left( \frac{\pi_\theta(\vec{z}^i|l)}{\pi_{\theta_{old}}(\vec{z}^i|l)} A_i, \text{clip} \left( \frac{\pi_\theta(\vec{z}^i|l)}{\pi_{\theta_{old}}(\vec{z}^i|l)}, 1 - \epsilon, 1 + \epsilon \right)  A_i \right) - \beta \mathbb{D}_{KL}\left(\pi_{\theta} || \pi_{ref}\right)\right) ,
\end{split}
\label{eq:GRPO-obj}
\]
\[
% \begin{equation}
    \mathbb{D}_{KL}\left(\pi_{\theta} || \pi_{ref}\right) = \frac{\pi_{ref}(\vec{m}^i|l)}{\pi_{\theta}(\vec{m}^i|l)}- \log\frac{\pi_{ref}(\vec{m}^i|l)}{\pi_{\theta}(\vec{m}^i|l)} - 1,
% \end{equation}
\]
where $\epsilon$ and $\beta$ are hyper-parameters, $\pi_{\theta_{ref}}$ is the reference policy, and $A_i$ is the advantage, computed using a group of rewards $\{r_1, r_2, \ldots, r_G\}$ corresponding to the outputs within each group:
\[
% \begin{equation}
    A_i = \frac{r_i - {\mathrm{mean}(\{r_1, r_2, \cdots, r_G\})}}{{\mathrm{std}(\{r_1, r_2, \cdots, r_G\})}}.
% \end{equation}
\]

\subsection{Motion Tracking Reward}

% 为了使得模型生成的motion可以应用到humanoid 上，需要如下操作： motion retargeting 以及 Motion Tracking Policy。

% To deploy the generated motions on a humanoid robot and obtain tracking rewards, two key steps are required: motion retargeting and a motion tracking policy.

To deploy the generated motions on a humanoid robot in the simulator to obtain tracking rewards, we formulate a three-stage process: motion retargeting, motion tracking policy training, and offline evaluation to obtain tracking rewards.

\subsubsection{Motion Retargeting}

% 由于人体和humanoid 在形态学上的差异，it is necessary to retarget the human motion into humanoid robot motion. Following h2o~\citep{he2024learning}, we employed an optimization-based approach to achieve this.

% Due to morphological differences between the human body and the humanoid robot, it is necessary to retarget human motion to humanoid-compatible motion. Following H2O~\citep{he2024learning}, we adopt an optimization-based approach to achieve this.

% Since the dataset consists entirely of human motion, the motion generator outputs human SMPL motion sequences. To apply these to a robot, it is necessary to retarget the human motion into robot motion. We employed an optimization-based approach to achieve this.

% \textbf{Optimization of human shape parameters \(\beta\).} %Since humans and humanoid robots have similar skeletons, we can track the human joint positions across frames and map them to the corresponding joints in a humanoid robot, resulting in humanoid keypoints \(P_{\text{robot}}\) for high-level control. The joint positions \(P_{\text{joints}}\) can be obtained via forward kinematics \(F_{\text{fk}}\):

Due to the morphological differences between the human body and humanoid robots, human motion needs to be re-adjusted to be compatible with humanoid robots. We follow the idea of H2O~\citep{he2024learning} and adopt an optimization-based approach to achieve the retargeting process.

% Specifically, we first use forward kinematics to calculate the keypoint position of the humanoid robot. Then the parameters of the SMPL model \citep{loper2023smpl} are gradient updated to fit the calculated keypoint position. This process ensures accurate retargeting and provides a basis for the subsequent learning of motion tracking policies.

Specifically, based on the morphological characteristics of the humanoid robot, we first optimized the body shape parameters $\bm{\beta}$ of the SMPL model through gradient descent to match the robot's geometric structure and establish the corresponding human body shape. Then, based on the fixed body shape, we iteratively adjusted the pose parameters $\bm{\theta}$ of the SMPL model by combining kinematic inverse solution with gradient optimization to make the human body model joint rotation match the robot's target posture, and finally achieved full body posture alignment based on keypoint position constraints. This hierarchical optimization strategy ensures physically reasonable motion retargeting effects by a priori decoupling body shape adaptation and posture migration.

% \begin{equation}
% P_{\text{joints}} = F_{\text{fk}}(P_{\text{human}}(\beta, \theta_{\text{root}})).
% \label{eq:3}
% \end{equation}

% Since humans have different shapes from humanoid robots, we first optimize the human shape parameters \(\beta\) to ensure that resized human shapes closely resemble those of a humanoid robot. Specifically, we first obtain joint positions of a humanoid robot under a standard standing pose: \(P^S_{\text{robot}}\). Then, under the same standing pose, we optimize \(\beta\) to make human joint positions \(P^S_{\text{joints}}\) the same as the corresponding humanoid joint positions \(P^S_{\text{robot}}\):
% % \[
% % \min_{\beta} \| P^S_{\text{joints}} - P^S_{\text{robot}} \|_2,
% % \]
% %     s.t.
% % \(
% % P^S_{\text{joints}} = F_{fk}(P_{\text{human}}(\beta, \theta^S_{\text{root}})),
% % \)

% \[
% \min_{\beta} \| P^S_{\text{joints}} - P^S_{\text{robot}} \|_2, s.t. P^S_{\text{joints}} = F_{\text{fk}}(P_{\text{human}}(\beta, \theta^S_{\text{root}})),
% \]
    


% where $\theta^S_{\text{root}}$ denotes the standing pose. 
% After that, we obtain the optimal \(\beta^*\) in \(P_{\text{human}}\), and following Eq.~\eqref{eq:3}, we can obtain the adjusted human joint positions \(P'_{\text{joints}}\). Finally, we directly set humanoid robot keyframes as the adjusted human joint positions:

% \[
% P_{\text{robot}} := P'_{\text{joints}}.
% \]

% \textbf{Solving humanoid motor DoF positions \(q_{\text{robot}}\)}. With the optimal \(\beta^*\), we need to extract the motor DoF positions \(q_{robot}\) through inverse kinematics with the loss \(\mathcal{L}_{ik}\):

% \begin{equation}
%     \mathcal{L}_{ik}(q_{\text{robot}}, s_{\text{root}}) = \| F_{\text{rk}}(q_{\text{robot}}, s_{\text{root}}) - P_{\text{robot}} \|_1.
%     \label{eq:lik}
% \end{equation}

% where \(s_{\text{root}}\) denotes robot root states including root translation and root orientation, \(F_\text{rk}\) denotes robot forward kinematics which maps from \(q_{\text{robot}}\), \(s_{\text{root}}\) to humanoid robot keypoint positions.


% \subsection{Motion Tracker: Perpetual Humanoid Controller (PHC) Method}

% In our approach, we adopt the Perpetual Humanoid Controller (PHC) framework to control physics-based humanoid robots for motion imitation and fail-state recovery. PHC is a goal-conditioned reinforcement learning method capable of handling noisy inputs from video estimates or language generation, achieving high-fidelity motion imitation on large-scale motion datasets, and naturally recovering from fail-states. Below, we provide a detailed description of this method, adapted to our specific implementation.

% \subsubsection{Problem Formulation}

% We formulate the motion imitation task as a Markov Decision Process (MDP), defined by the tuple \(\mathcal{M} = \langle \mathcal{S}, \mathcal{A}, \mathcal{T}, \mathcal{R}, \gamma \rangle\), where:
% - \(\mathcal{S}\) is the state space;
% - \(\mathcal{A}\) is the action space;
% - \(\mathcal{T}\) is the state transition dynamics;
% - \(\mathcal{R}\) is the reward function;
% - \(\gamma\) is the discount factor.

% The state \(s_t \in \mathcal{S}\) consists of the humanoid's proprioception \(s_t^p = (q_t, \dot{q}_t, \beta)\) and the goal state \(s_t^g\), where \(q_t\) denotes the pose, \(\dot{q}_t\) denotes the velocity, and \(\beta\) represents optional body shape parameters. For rotation-based motion imitation, the goal state is defined as:
% \[
% s_t^g = (\hat{\theta}_{t+1} \ominus \theta_t, \hat{p}_{t+1} - p_t, \hat{v}_{t+1} - v_t, \hat{\omega}_t - \omega_t, \hat{\theta}_{t+1}, \hat{p}_{t+1}),
% \]
% where \(\hat{\theta}_{t+1}\) and \(\hat{p}_{t+1}\) are the reference joint rotations and positions at the next time step, respectively, and \(\ominus\) denotes the rotation difference. For keypoint-based imitation, the goal state simplifies to:
% \[
% s_t^g = (\hat{p}_{t+1} - p_t, \hat{v}_{t+1} - v_t, \hat{p}_{t+1}).
% \]
% The action \(a_t \in \mathcal{A}\) specifies the target for the proportional-derivative (PD) controllers at each joint of the humanoid.

% The reward function is defined as:
% \[
% r_t = 0.5 r_t^g + 0.5 r_t^{\text{amp}} + r_t^{\text{energy}},
% \]
% where \(r_t^g\) is the task reward (for imitation or recovery), \(r_t^{\text{amp}}\) is the Adversarial Motion Prior (AMP) reward ensuring natural motion, and \(r_t^{\text{energy}}\) is an energy penalty term. For motion imitation, the task reward is:
% \begin{equation}
% \begin{aligned}
% & r_t^g = R^{\text{imitation}}(s_t, \hat{q}_{t+1}) = w_{\text{jp}} e^{-100 \|\hat{p}_t - p_t\|} \\
% & + w_{\text{jr}} e^{-10 \|\hat{q}_t \ominus q_t\|} + w_{\text{jv}} e^{-0.1 \|\hat{v}_t - v_t\|} + w_{\text{j}\omega} e^{-0.1 \|\hat{\omega}_t - \omega_t\|}
% \end{aligned}
% \end{equation}
% with weights \(w_{\text{jp}}, w_{\text{jr}}, w_{\text{jv}}, w_{\text{j}\omega}\) balancing the components. We train the policy \(\pi_{\text{PHC}}\) using Proximal Policy Optimization (PPO) combined with an AMP discriminator.

% % \subsubsection{Policy Architecture}

% % In the full PHC method, the policy \(\pi_{\text{PHC}}\) employs a Progressive Multiplicative Control Policy (PMCP), training multiple primitives via a Progressive Neural Network (PNN) and combining them using a Multiplicative Control Policy (MCP). Specifically, PMCP incrementally trains primitives \(P^{(1)}, P^{(2)}, \dots, P^{(K)}\) to learn increasingly difficult motion sequences, freezing each primitive before adding the next to avoid catastrophic forgetting. A composer \(C\) is then trained to dynamically combine these primitives.

% % In our implementation, however, we do not employ progressive learning. Instead, we train the policy \(\pi_{\text{PHC}}\) on the entire motion dataset in a single phase. The policy consists of multiple primitive networks \(P^{(1)}, P^{(2)}, \dots, P^{(K)}, P^{(F)}\), where \(P^{(1)}\) to \(P^{(K)}\) are for motion imitation, and \(P^{(F)}\) is for fail-state recovery. Each primitive \(P^{(k)}\) is a Gaussian policy:
% % \[
% % P^{(k)}(a_t | s_t) = \mathcal{N}(\mu^{(k)}(s_t), \sigma),
% % \]
% % where \(\mu^{(k)}(s_t)\) is the mean computed by a neural network, and \(\sigma\) is a fixed variance. A composer \(C(w_{1:K+1} | s_t)\) outputs a weight vector \(w_{1:K+1}\) to combine these primitives via MCP. The overall policy distribution is a Gaussian with mean and variance computed as:
% % \[
% % \mu_j(s_t) = \frac{\sum_{i=1}^{K+1} C_i(s_t) \mu_j^{(i)}(s_t) / \sigma_j^{(i)}(s_t)}{\sum_{i=1}^{K+1} C_i(s_t) / \sigma_j^{(i)}(s_t)}, \quad \sigma_j(s_t) = \left( \sum_{i=1}^{K+1} \frac{C_i(s_t)}{\sigma_j^{(i)}(s_t)} \right)^{-1},
% % \]
% % where \(j\) denotes the action dimension.

% \subsubsection{Training Procedure}

% Our training process comprises the following steps:
% \begin{enumerate}
%     \item \textbf{Imitation Primitive Training}: We simultaneously train \(K\) imitation primitives \(P^{(1)}, \dots, P^{(K)}\) on the entire motion dataset using the imitation reward \(R^{\text{imitation}}\). Unlike the original PHC method, which uses hard-negative mining to progressively train on harder sequences, we train on the full dataset in one go.
%     \item \textbf{Fail-State Recovery Primitive Training}: The fail-state recovery primitive \(P^{(F)}\) is trained separately on a subset of simple locomotion data (e.g., walking and running), using a modified state space (retaining only root reference information) and a point-goal reward \(R^{\text{recover}}\).
%     \item \textbf{Composer Training}: The composer \(C\) is trained with mixed experiences from imitation and recovery tasks to dynamically combine all primitives.
% \end{enumerate}

% During inference, the policy \(\pi_{\text{PHC}}\) dynamically combines the primitives based on the current state via the composer, generating an action distribution. This approach retains the PHC's advantage of using multiple primitives and MCP, supporting parallel processing of motion imitation and fail-state recovery. However, without progressive training, our implementation may encounter some forgetting issues, particularly with diverse motions.

\subsubsection{Motion Tracking Policy Training}
\label{sec:motion_tracking}
% 经过retargeting之后的motion在形态学上与humanoid robot一致，借助预先训练好的motion tracker policy，可以在仿真器中部署并迁移到真实环境。我们参考了exbody2~\citep{ji2024exbody2}的方法, dopts a two-stage teacher-student training procedure，在amass数据集上训练一个通用的、可以迁移到真实环境的 motion tracker policy。Specifically, the oracle teacher policy is first trained with an off-the-shelf reinforcement learning (RL) algorithm, PPO~\citep{schulman2017proximal}, with privileged information that can be obtained only in simulators. For the second stage, we remove the privileged information with observations which are not available with the real world, and distill the teacher policy to a deployable student policy. We train our policies using IsaacGym~\citep{makoviychuk2021isaac} with efficient parallel simulation.

After retargeting, the motion is morphologically consistent with the humanoid robot. With a pre-trained motion tracking policy, it can be deployed in the simulator and transferred to the real world to verify the tracking performance for any given motion. Inspired by Exbody2~\citep{ji2024exbody2}, we adopt a two-stage teacher-student training procedure to train a general motion tracking policy on the AMASS~\citep{mahmood2019amass} dataset. Specifically, the oracle teacher policy is first trained using the off-the-shelf reinforcement learning algorithm PPO~\citep{schulman2017proximal}, utilizing privileged information available only in the simulator. For the second stage, we remove the privileged information with observations that are not available in the real world, and distill the teacher policy into a deployable student policy. We train our policies using IsaacGym~\citep{makoviychuk2021isaac}, leveraging its efficient parallel simulation capabilities.

\textbf{Stage 1: Teacher Policy Training.}
The teacher policy $\hat{\pi}$ is trained as an oracle in simulation using PPO. It uniquely leverages privileged information $p_t$ inaccessible in the real world, such as ground-truth root velocity, joint global positions, and environmental physical properties (e.g., friction coefficients, motor strength). This is combined with proprioceptive states $o_t$ and motion tracking targets $g_t$. The objective of the teacher policy is to maximize the expectation of accumulated rewards by outputting target joint positions $\hat{a}_t \in \mathbb{R}^{23}$ for Proportional Derivative (PD) controllers, encouraging accurate tracking of motion demonstrations along with robust behavior. 
This process yields a high-performing expert policy that benefits from comprehensive data from simulation only.

\textbf{Stage 2: Student Policy Training.} The student policy $\pi$ is trained to mimic the teacher policy but without access to privileged information, making it suitable for real-world deployment. It takes a history of past real-world history observations $o_{t-H:t}$ along with the motion target $g_t$ as input to predict actions $a_t$. The training follows a DAgger-like~\citep{ross2011reduction} strategy: The student policy is rolled out in the simulation environment to generate training data. For each visited state, the teacher policy $\hat{\pi}$ computes the oracle action $\hat{a}_t$ which serves as the supervision signal. The student policy is then refined by iteratively minimizing an MSE loss, defined as $l = \Vert a_t - \hat{a}_t \Vert^2$, on the accumulated data until the loss converges. A critical aspect is preserving a sufficiently long sequence of historical observations for effective learning.

% \subsubsection{Motion Tracking Reward Design}
\subsubsection{Offline Evaluation}

Upon acquiring a student policy with demonstrated generalization capability, we rigorously evaluate its performance within the training simulator (e.g., IsaacGym). The policy's motion tracking performance is quantified using task-specific success rates, which subsequently serve as motion tracking rewards to fine-tune the motion generator through an iterative optimization process, denoted as:
\[
R_{tracking}^{m_i}=\mathbb{I}\left( \textbf{Succ}(\pi, m_i) \right),
\]
where $\pi$ denotes the student policy pre-trained in Section \ref{sec:motion_tracking}, $m_i$ represent the $i$-th retargeted motion, and $ \textbf{Succ}(\pi, m_i) $ is a binary success indicator for whether policy $\pi$ successfully completes the motion tracking task for $m_i$. The task completion criteria are defined based on motion quality metrics, where failure conditions include positional deviation exceeding a predefined threshold $\epsilon$, and loss of body balance.



\subsection{Alignment Verification Module}

We perform RL optimization using the pre-trained motion tracking policy in Section \ref{sec:motion_tracking}, aiming to generate motion sequences that are easier for the tracking policy to follow. However, relying solely on this objective may cause the generated motions to deviate from the input textual instructions. 
To address this issue, we propose an \textbf{Alignment Verification Module} to regularize the motion generator, ensuring that the generated motions maintain semantic correspondence while being significantly more physically plausible.
% To address this issue, we propose an \textbf{Alignment Verification Module} to regularize the motion generator, 
% ensuring that the generated motions remain semantic correspondence while much more physically feasible
% ensuring that the generated motions remain feasible while faithfully adhering to the input instructions.	

Specifically, we propose implementing the Alignment Verification using contrastively pre-trained motion and text encoders. It consists of a motion encoder $E_m$ and a text encoder $E_t$, both trained with the following objective:
\[
\mathcal{L}_{CL} = (1 - y) (\| \mathbf{f_t} - \mathbf{f_m}\|)^2 + y (max(0, m - \| \mathbf{f_t} - \mathbf{f_m}\|))^2,
\]
where $y$ is a binary label indicating the matched text-motion pairs and $m$ is the manually set margin. $\mathbf{f_t} = E_t(\mathbf{t})$ and $\mathbf{f_m} = E_m(\mathbf{m})$ are embeddings extracted by text and motion encoders, respectively.

$E_t$ and $E_m$ map the text and motion modalities into a shared embedding space, where semantically similar textual descriptions and motion sequences have smaller Euclidean distances. 
We propose two implementations: the \textbf{motion alignment verification} and the \textbf{text alignment verification}, which measure the distance between the input text and the generated motion, and between the ground-truth motion and the generated motion, respectively,
\[
R_{TA}^{m_i} = (\| \mathbf{E_t(\mathbf{t})} - \mathbf{E_m(\mathbf{m_{pred}})}\|)^2, \,\, R_{MA}^{m_i} = (\| \mathbf{E_m(\mathbf{m})} - \mathbf{E_m(\mathbf{m_{pred}})}\|)^2,
\]
where $R_{TA}^{m_i}$ indicates the text alignment verification, $R_{MA}^{m_i}$ indicates the motion alignment verification, and $m_{pred}$ indicates the generated motion, respectively.

% \subsection{Reward Setting}

% \subsubsection{Physically plausible reward: PHC as reward}

% For our motion generator training, we utilize trained PHC policy as a reward function to judge the quality of generated motions. We use the task reward \(r_t^g\) as the physically plausible reward, which reflects the practical capabilities of generated motion.

% % \begin{equation}
% % r_t^g = R^{\text{imitation}}(s_t, \hat{q}_{t+1}) = w_{\text{jp}} e^{-100 \|\hat{p}_t - p_t\|} + w_{\text{jr}} e^{-10 \|\hat{q}_t \ominus q_t\|} + w_{\text{jv}} e^{-0.1 \|\hat{v}_t - v_t\|} + w_{\text{j}\omega} e^{-0.1 \|\hat{\omega}_t - \omega_t\|},
% % \end{equation}

% % \begin{equation}
% % \begin{split}
% % r_t^g = R^{\text{imitation}}(s_t, \hat{q}_{t+1}) &= w_{\text{jp}} e^{-100 \|\hat{p}_t - p_t\|} \\
% % &\quad + w_{\text{jr}} e^{-10 \|\hat{q}_t \ominus q_t\|} + w_{\text{jv}} e^{-0.1 \|\hat{v}_t - v_t\|} + w_{\text{j}\omega} e^{-0.1 \|\hat{\omega}_t - \omega_t\|}
% % \end{split}
% % \end{equation}

% \begin{equation}
% \begin{aligned}
% & r_t^g = R^{\text{imitation}}(s_t, \hat{q}_{t+1}) = w_{\text{jp}} e^{-100 \|\hat{p}_t - p_t\|} \\
% & + w_{\text{jr}} e^{-10 \|\hat{q}_t \ominus q_t\|} + w_{\text{jv}} e^{-0.1 \|\hat{v}_t - v_t\|} + w_{\text{j}\omega} e^{-0.1 \|\hat{\omega}_t - \omega_t\|}
% \end{aligned}
% \end{equation}

% \subsubsection{Alignment Discriminator Module}

% We perform reinforcement learning (RL) optimization using a motion tracking policy, aiming to generate motion sequences that are easier for the tracking policy to follow. However, relying solely on this objective may cause the generated motions to deviate from the input textual instructions.	To address this issue, we propose an Alignment Discriminator to regularize the motion generator, ensuring that the generated motions remain feasible while faithfully adhering to the input instructions.	

% Specifically, we propose implementing the Alignment Discriminator using contrastively pre-trained motion and text encoders. It consists of a motion encoder $E_m$ and a text encoder $E_t$, both trained with the following objective:

% \begin{equation}
% \mathcal{L}_{CL} = (1 - y) (\| \mathbf{f_t} - \mathbf{f_m}\|)^2 + y (max(0, m - \| \mathbf{f_t} - \mathbf{f_m}\|))^2,
% \end{equation}

% where $y$ is a binary label indicating the matched text-motion pairs and $m$ is the manually set margin. $\mathbf{f_t} = E_t(\mathbf{t})$ and $\mathbf{f_m} = E_m(\mathbf{m})$ are embeddings extracted by text and motion encoders, respectively.

% $E_t$ and $E_m$ map the text and motion modalities into a shared embedding space, where semantically similar textual descriptions and motion sequences have smaller Euclidean distances. 
% We propose two implementations: the motion alignment discriminator and the text alignment discriminator, which measure the similarity between the input text and the generated motion, and between the ground-truth motion and the generated motion, respectively.


% 中文

% 利用motion tracking policy 进行 RL 优化，模型的优化目标是生成对于tracking policy而言更容易track的motion序列。然而，仅有这一个优化目标会使得模型输出的motion偏离输入的文本指令。为了解决这个问题，我们提出了Alignment Discriminator来约束motion generator的行为，让模型生成更加feasible的motion的同时保持模型生成的准确性。

% Specifically，we propose 使用 contrastive pre-trained motion and text 实现 Alignment Discriminator, which consists of contrastive pre-trained motion encoder $E_m$ and text encoder $E_t$,  which are trained with the following objective:

% \begin{equation}
% \mathcal{L}_{CL} = (1 - y) (\| \mathbf{f_t} - \mathbf{f_m}\|)^2 + y (max(0, m - \| \mathbf{f_t} - \mathbf{f_m}\|))^2,
% \end{equation}

% where $y$ is a binary label indicating the matched text-motion pairs and $m$ is the manually set margin. $\mathbf{f_t} = E_t(\mathbf{t})$ and $\mathbf{f_m} = E_m(\mathbf{m})$ are embeddings extracted by text and motion encoders, respectively.

% $E_t$ and $E_m$ map the text and motion modality into a shared embedding space, where semantically similar textual descriptions and motion sequences exhibit smaller Euclidean distances. 我们提出了两种实现方式: motion alignment discriminator and text alignment discriminator, 分别表示输入的text和生成的motion之间的度量、ground truth motion和生成的motion之间的度量。
% which 计算输入的text与生成的motion之间的度量，而ground-truth motion-motion alignment discriminator计算数据集中ground truth motion和生成的motion之间的度量 respectively.


% Semantic Conformance Discriminator (SCD)
% Semantic: 强调语义层面的匹配。
% Conformance: 强调与文本指令的符合、一致性。
% Cross-Modal Semantic Alignment Verifier (CSAV)
% Cross-Modal: 点出文本和运动是不同模态。
% Semantic Alignment: 强调语义上的对齐。
% Verifier: 听起来比Discriminator更侧重于验证准确性。
% Instructional Fidelity Modulator (IFM)
% Instructional: 指代输入的文本指令。
% Fidelity: 强调生成运动对指令的忠实度。
% Modulator: 暗示它调整生成器的行为。
% Textual Coherence Guardian (TCG)
% Textual Coherence: 强调与文本的连贯性和一致性。
% Guardian: 守护者，比喻其约束作用，更生动。

% Referential Kinematic Fidelity Discriminator (RKFD)
% Referential: 指代以Ground-truth为参考。
% Kinematic Fidelity: 强调运动学上的保真度和真实感。
% Motion Realism Adherence Discriminator (MRAD)
% Motion Realism: 强调生成运动的真实感。
% Adherence: 强调与真实运动的贴合程度。
% Intrinsic Motion Conformity Assessor (IMCA)
% Intrinsic Motion: 指代运动本身的特性，源自Ground-truth。
% Conformity Assessor: 符合性评估器，听起来更专业。
% Authentic Motion Structure Verifier (AMSV)
% Authentic Motion: 强调真实运动。
% Structure Verifier: 验证生成运动是否具有真实运动的结构特征。


% 我们使用了off-the-shell text-motion retrieval model, 利用模型学到的text和motion共享的feature space空间上的feature的距离提供discrimination。我们使用了两种变体：d
% ground truth motion

% In order to prevent the model from only generating simple motions that are easy to track, we also use text motion alignment rewards to guide the motion generated by the model to be consistent with the text.

% To this end, we propose to design the reward function using contrastive pre-trained motion and text encoders. Specifically, we adopt the motion and text encoders in HumanML3d, which are trained with the following objective:

% \begin{equation}
% \mathcal{L}_{CL} = (1 - y) (\| \mathbf{f_t} - \mathbf{f_m}\|)^2 + y (max(0, m - \| \mathbf{f_t} - \mathbf{f_m}\|))^2,
% \end{equation}
% where $y$ is a binary label indicating the matched text-motion pairs and $m$ is the manually set margin. $\mathbf{f_t} = E_t(\mathbf{t})$ and $\mathbf{f_m} = E_m(\mathbf{m})$ are embeddings extracted by text and motion encoders, respectively.

% $E_t$ and $E_m$ map the text and motion modality into a shared embedding space, where semantically similar textual descriptions and motion sequences exhibit smaller Euclidean distances. Given a textual description $\mathbf{t}$ and the generated motion $\mathbf{m}_{\mathrm{pred}}$ conditioned on $\mathbf{t}$, we can thus design the reward function as follows:
% \begin{equation}
%     \label{eq:motion_padding}
%     r (\mathbf{t}, \mathbf{m}) = \left\{
%     \begin{array}{ll}
%     - \lambda_t \| \mathbf{f}_{\mathbf{t}} - \mathbf{f}_{\mathbf{m}_{\mathrm{pred}}}\|^2, & {\text{text-only}} \\
%     - \lambda_t \| \mathbf{f}_{\mathbf{t}} - \mathbf{f}_{\mathbf{m}_{\mathrm{pred}}}\|^2 - \lambda_m \| \mathbf{f}_{\mathbf{m}_{\mathrm{gt}}} - \mathbf{f}_{\mathbf{m}_{\mathrm{pred}}}\|^2, & \text{paired}
%     \end{array}
%     \right.
%     ,
% \end{equation}
